Two Methods For Wild Variational Inference

Variational inference provides a powerful tool for approximate probabilistic in- ference on complex, structured models. Typical variational inference methods, however, require to use inference networks with computationally tractable proba- bility density functions. This largely limits the design and implementation of vari- ational inference methods. We consider wild variational inference methods that do not require tractable density functions on the inference networks, and hence can be applied in more challenging cases. As an example of application, we treat stochastic gradient Langevin dynamics (SGLD) as an inference network, and use our methods to automatically adjust the step sizes of SGLD, yielding significant improvement over the hand-designed step size schemes

==> experiment.tex <==

%Figure ~\ref{} - \ref{} show the result of our SteinGAN. 
\section{Empirical Results}  \label{sec:gan}

We evaluated our SteinGAN on four datasets,  
MNIST, CIFAR10, CelebA \citep{liu2015faceattributes}, and Large-scale Scene Understanding (LSUN) \citep{yu2015lsun}, on which we find our method tends to generate realistic-looking images competitive with, sometimes better than DCGAN \citep{radford2015unsupervised} (see Figure~\ref{fig:face}-Figure~\ref{fig:cifar10}). 
% mnist \footnote{\url{http://yann.lecun.com/exdb/mnist/}}
% cifar10 \footnote{\url{https://www.cs.toronto.edu/~kriz/cifar.html}}
% celeba  \footnote{\url{http://mmlab.ie.cuhk.edu.hk/projects/CelebA.html}}
% lsun \footnote{\url{http://lsun.cs.princeton.edu/2016/}}
%In particular, we find we generate better images than DCGAN on CelebA (Figure~\ref{fig:face}), and our simulated CIFAR10 images achives better testing classification accuracy when used as a training data (see Figure~\ref{fig:cifar10}). 
%generative adversarial networks. 
%See Appendix~\ref{sec:gan} for more information. 
We will provide code to reproduce our experiments. 


%\subsection{Implementation}
\newcommand{\enc}{\mathrm{E}}
\newcommand{\dec}{\mathrm{D}}
\paragraph{Model Setup} In order to generate realistic-looking images, we define our energy model based on an autoencoder: 
\begin{align}\label{equ:px}
%p(x|\theta) \propto \exp(-\phi(x,\theta)),~~~~~ \text{where~~~~}  \phi(x, \theta) = \alpha || x -   dec(enc(x))  |, 
p(x|\theta) \propto \exp(-  || x -   \dec(\enc(x;~ \theta);~\theta) ||), 
\end{align}
where $x$ denotes the image. 
This choice is motivated by Energy-based GAN \citep{zhao2016energy} in which the autoencoder loss is used as a discriminator but without a probabilistic interpretation. 
We assume $f(\eta;~\xi)$ to be a neural network whose input $\xi$ is a $\dilincheck{100}$-dimensional random vector drawn by $\mathrm{Uniform}([0,1])$. 
The positive definite kernel in SVGD is defined by the RBF kernel on the hidden representation obtained by the autoencoder in \eqref{equ:px}, that is, 
$$
k(x, x') = \exp(-\frac{1}{h^2} ||\enc(x;~\theta) - \enc(x';~\theta)||^2). 
$$
As we discussed in Section~\ref{sec:amortizedsvgd}, the kernel provides a repulsive force to encourage diversity on the generated samples. % via the term $\nabla_x k(x,x')$ in \eqref{equ:update11}. 
This is similar to the heuristic ``repelling regularizer'' in \citep{zhao2016energy}, but is derived in a principled way. 
We take the bandwidth to be $h = \red{0.5}\times \mathrm{med}$, where $\mathrm{med}$ is the median of distances between $\enc(x)$ on image simulated by $f(\eta;~ \xi)$. 
This makes the kernel change adaptively based on both $\theta$ (through $\E(x;~\theta)$) and $\eta$ (through bandwidth $h$). 

%For MNIST and CIFAR-10, each image $x$ also has a discrete label $y$, and we train a joint model on $(x,y)$:
Some datasets include both images $x$ and 
their associated discrete labels $y$. We train a joint energy model on $(x,y)$ 
to capture both the inner structure of the images and its predictive relation with the label, which allows us to simulate images 
with a control on which category it belongs to. Our model joint energy model is defined to be 
%conditional on each categorial. 
\begin{align}\label{equ:pxy}
p(x, y|\theta) \propto \exp\big (-  || x -   \dec(\enc(x;~\theta);~\theta) || - \beta \max(m,~\sigma(y, ~ \enc(x;~\theta)))\big ),  %\red{dilin: square?}
\end{align}
where $\sigma(\cdot,\cdot)$ is the cross entropy loss function of a fully connected output layer. 
In this case, our generative network will first draw a $y$ randomly according to the empirical counts in the dataset, 
and pass it into a neural network together with a $100$ dimensional random vector $\xi$ to generate image $x$. 
This allows us to generate images for particular categories by controlling the value of input $y$. 
We set $\beta=\dilincheck{?}$ and $m$ by \dilincheck{?}. 
%where $\sigma$ denotes  a fully connected layer.  

\paragraph{Regularization}
In practice, we find it is useful to modify \eqref{equ:updatetheta} to be 
$$
\theta \gets \theta - \hat\E_{obs}[ \nabla_\theta \phi (x,\theta) ] + 
(1-\gamma) \hat\E_{\eta} [\nabla_\theta f(x, \theta)]. 
$$
where $\gamma$ is a discount factor (we take $\gamma = 0.7$). 
%This is equivalent to MAP of $\theta$ with a conjugate prior: %
This is equivalent to maximizing a regularized likelihood: 
$$
\max_\theta  \{ \log   p(x |\theta)  +  \gamma \Phi(\theta)\}
$$
where $\Phi(\theta)$ is the log-partition function and note that $\exp( \gamma \Phi(\theta))$ is a conjugate prior of $p(x|\theta)$. 

We also stabilize the algorithm by .xxxx. 

\begin{comment}
We tested our SteinGAN on four datasets,  
MNIST \footnote{\url{http://yann.lecun.com/exdb/mnist/}}, CIFAR10 \footnote{\url{https://www.cs.toronto.edu/~kriz/cifar.html}}, CelebA \footnote{\url{http://mmlab.ie.cuhk.edu.hk/projects/CelebA.html}}, and Large-scale Scene Understanding (LSUN) \footnote{\url{http://lsun.cs.princeton.edu/2016/}}, on which we find our method tends to generate realistic-looking images competitive with DCGAN \citep{radford2015unsupervised} (see Figure~\ref{fig:face}-Figure~\ref{fig:cifar10}). 
In particular, we find we generate better images than DCGAN on CelebA (Figure~\ref{fig:face}), 
and our simulated CIFAR10 images achives better testing classification accuracy when used as a training data (see Figure~\ref{fig:cifar10}). 
%generative adversarial networks. 
See Appendix~\ref{sec:gan} for more information. 
We will provide code to reproduce our experiments.  
\end{comment}


\subsection{MNIST}
The MNIST database of handwritten digits has a training set of $60,000$ examples. 
% Our discriminator has 3 layers for both encoder and decoder with shared parameters. 
Both DCGAN and our model produce high quality images, samples are indistinguishable from dataset images.
\begin{figure}[htb]
\centering
\begin{tabular}{cc}
\includegraphics[width=0.3\textwidth]{\dilinfig/mnist/dcgan_mnist.png} & 
\includegraphics[width=0.3\textwidth]{\dilinfig/mnist/mnist_steingan.png}   \\
%\includegraphics[width=0.2\textwidth]{\dilinfig/mnist/vgd_gan_small.png} \\
DCGAN & SteinGAN \\
\vspace{5\baselineskip}
\end{tabular}
\begin{comment}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{|l|c|c|c|}
\hline
Training Data & Real Images & DCGAN %& SteinGAN (w/o kernel) 
& SteinGAN \\
\hline
Testing Accuracy& 92.58 \% &  41.82 \%  %& 62.93 \% 
& 58.69 \%\\
\hline
\end{tabular}
\end{comment}
\caption{
 MNIST images generated by DCGAN and our SteinGAN conditional on each digit. We use the joint model in \eqref{equ:pxy} to allow us generate images for each digit. 
%Upper: MNIST images generated by DCGAN and our SteinGAN conditional on each digit. We use the joint model in \eqref{equ:pxy} to allow us generate images for each digit. Lower: Testing accuracy when using simulated images (of the same size as the real training set) to train ResNets for classification. SteinGAN achieves higher testing accuracy than DCGAN.
}
\label{fig:mnist}
\end{figure}


\subsection{CIFAR-10}
CIFAR-10 is very diverse, and with only 50,000 training examples.

We first evaluate the inception score for all models.
We propose to use the samples to train a classifer and test on the real testing images, which, none of the GAN models saw before during the learning stage. Our SteinGAN achieves higher accuracy.

\begin{figure}[t]
\centering
\begin{tabular}{ccc}
\raisebox{8.3em}{
\renewcommand{\arraystretch}{1.5}
\newcommand{\tmpfnt}{\small}
\hspace{-.04\textwidth}
\begin{tabular}{r}
\tmpfnt airplane \\
\tmpfnt automobile \\
\tmpfnt bird \\
\tmpfnt cat \\
\tmpfnt deer \\
\tmpfnt dog \\
\tmpfnt frog \\
\tmpfnt horse \\
\tmpfnt ship \\
\tmpfnt truck
\end{tabular}} & 
\hspace{-.04\textwidth}\includegraphics[width=.42\textwidth]{\dilinfig/cifar10/dcgan_cifar10.png}  & 
%\includegraphics[width=.3\textwidth]{\dilinfig/cifar10/vgd_no_kernel_cifar10.png}  & 
\includegraphics[width=.42\textwidth]{\dilinfig/cifar10/vgd_cifar10.png}  \\
& DCGAN 
%& SteinGAN (w/o kernel) 
& SteinGAN \\
\vspace{5\baselineskip}
\end{tabular}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{|l|c|c|c|c|}
\hline
\multicolumn{5}{|c|}{Inception Scores} \\
\hline
 & Real Images & 500 Duplicate  & DCGAN  & SteinGAN \\
\hline
ImageNet & 11.237 & 11.100 & 6.581 & 6.209 \\
\hline
Cifar10 & 9.848 & 9.807 & 7.193 & 7.065 \\
\hline
\end{tabular}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{|c|c|c|c|}
\hline
\multicolumn{4}{|c|}{Testing Accuracy} \\
\hline
Real Images & 500 Duplicate  & DCGAN  & SteinGAN \\
\hline
92.58 \% &  44.96 \% & 44.78 \%  & 63.89 \%\\
\hline
\end{tabular}
\vspace{5\baselineskip}
\caption{Result on CIFAR-10. ``500 Duplicate'': we randomly select 500 images from the training set and duplicate the selected set 100 times.
Upper: Images simulated by DCGAN and SteinGAN (based on joint model \eqref{equ:pxy}) for each category. 
Middle: Inception scores for samples generated by various models for 50,000 images on inception model trained on both ImageNet and Cifar10. 
Lower: Testing accuracy when using simulated images (of the same size as the real training set) to train ResNets for classification. SteinGAN achieves higher testing accuracy than DCGAN.}%even though the images on in the upper panel look almost equally good visually.}
\label{fig:cifar10}
\end{figure}


\begin{figure}[t]
\centering
\begin{tabular}{cc}
\includegraphics[width=0.45\textwidth]{\dilinfig/faces/dcgan_bright.png} & 
\includegraphics[width=0.45\textwidth]{\dilinfig/faces/vgd_faces_small.png} \\
DCGAN & SteinGAN \\
\end{tabular}
\begin{tabular}{c}
\includegraphics[width=0.85\textwidth]{\dilinfig/faces/z2.pdf} \\
\end{tabular}
\caption{Results on CelebA. Upper: Images generated by DCGAN and our SteinGAN. Lower: images generated by SteinGAN when performing a random walk $\xi\gets \xi + 0.01\times\mathrm{Uniform}([-1,1])$ on the random input $\xi$. It can be observed that a generation of a man with glasses is gradually changed to a woman with blonde hair, all of which make a lot of sense.}
\label{fig:face}
\end{figure}


\begin{figure}[t]
\centering
\begin{tabular}{cc}
\includegraphics[width=0.45\textwidth]{\dilinfig/lsun/dcgan_5_7.png} & 
\includegraphics[width=0.45\textwidth]{\dilinfig/lsun/vgd_5_7.png} \\
DCGAN & SteinGAN\\
\end{tabular}
\caption{Images generated by DCGAN and our SteinGAN on LSUN.}
\label{fig:room}
\end{figure}



\begin{figure}[h]
\centering
\includegraphics[width=0.9\textwidth]{\dilinfig/faces/vgd_gan-20.png}  
\caption{More images generated by SteinGAN on CelebA.}
\label{fig:facemore}
\end{figure}


